Progressive Evolution from Single-Point to Polygon for Scene Text

The advancement of text shape representations towards compactness has enhanced text detection and spotting performance, but at a high annotation cost. Current models use single-point annotations to reduce costs, yet they lack sufficient localization information for downstream applications. To overcome this limitation, we introduce Point2Polygon, which can efficiently transform single-points into compact polygons. Our method uses a coarse-to-fine process, starting with creating and selecting anchor points based on recognition confidence, then vertically and horizontally refining the polygon using recognition information to optimize its shape. We demonstrate the accuracy of the generated polygons through extensive experiments: 1) By creating polygons from ground truth points, we achieved an accuracy of 82.0% on ICDAR 2015; 2) In training detectors with polygons generated by our method, we attained 86% of the accuracy relative to training with ground truth (GT); 3) Additionally, the proposed Point2Polygon can be seamlessly integrated to empower single-point spotters to generate polygons. This integration led to an impressive 82.5% accuracy for the generated polygons. It is worth mentioning that our method relies solely on synthetic recognition information, eliminating the need for any manual annotation beyond single points.

==> sec/0_abstract.tex <==
\begin{abstract}
In recent years, text detection has attracted considerable attention due to its diverse applications. However, the significant cost associated with annotations remains a notable challenge. Although existing methods suggest cost mitigation through the utilization of single points for scene text spotting, this approach may prove inadequate in certain applications, such as scene text editing, where relying solely on a single point to convey text location information is insufficient. To address this challenge, our paper introduces an innovative point-to-polygon text detection method capable of generating polygons based solely on point and text content annotations. Specifically, we present a multi-granularity recognition-guided generation that leverages recognition information to transform points into polygons. The process begins by generating coarse anchors from points using a Recognition Confidence Guided schedule (RCG), which produces a series of anchors and subsequently selects the optimal one. Following this, we employ a Recognition Loss Guided schedule (RLG) that utilizes recognition loss to align anchor boundary points with the text. Lastly, given that the polygon generated from the RLG typically exceeds the length of the text, we introduce a Recognition Attention guided (RAG) schedule that effectively removes superfluous points. Extensive experiments demonstrate the effectiveness and potential of the proposed Point2Polygon.

\end{abstract}

% 4个与图片长宽比相近的不同大小矩形框，大小分别为原图的1/5、1/8、10/1、1/30用于处理不同大小的字符数适中文本实例，2个近似正方形框，边长为宽的1/20、1/30，用于处理含字符数较少的文本实例，2个狭长的长矩形框，宽分别为原图宽的1/20、1/10，分别为原图长的1/25、1/8,用于处理含字符数较多的长文本实例

==> sec/1_intro.tex <==
% \section{Introduction}
% \label{sec:intro}

% % 1. Text Detection(application and issue).
% % 2. history(Box--Polygon--Point).
% % 3. Point: Box \cite{}.
% % 4. Therefore, we introduce .......(Module) 
% % 5. Contribution.
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{fig/intro.pdf}
%     \caption{ (a) Downstream tasks that require rectangular boxes. (b) Our proposed method.
%     }
%     \label{fig:intro}
% \end{figure}

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/related.png}
%     \caption{ Distinct stage of text detection.
%     }
%     \label{fig:related}
% \end{figure*}

% Scene Text Detection is a fundamental task for many downstream real-world applications, which enables machines to extract positional information about the rich text presented in the scene. Although the field of scene text detection has witnessed remarkable progress in recent years, enabling many real-world applications such as document digitization, document scanning, and text editing, the significant cost associated with annotation in order to address the variability of scene text shapes remains a significant challenge.

% Efforts to accurately predict text of varying forms have evolved over time. In the 1990s, the annotation of text shapes was confined to horizontal rectangular boxes, tailored for horizontal text. Fast forward to 2010, the introduction of rotating rectangular boxes marked a breakthrough for multi-directional text. Subsequently, in 2017, the quest for precision led to the adoption of quadrilateral and polygonal boxes, aimed at encapsulating the complexity of arbitrary shapes. However, at the same time, the cost of annotation has become more and more expensive, and the difficulty of obtaining large-scale annotated data has led to a decrease in the generalization performance of the model. Until SPTS~\cite{peng2022spts} proposes to characterize text shapes with a minimal and efficient single point, which greatly improves the efficiency of text location annotation.

% While single-point annotation has certainly made strides in the right direction, some challenges persist in certain downstream tasks. Taeho Kil~\cite{kil2023towards} \etal suggest that point annotation is not sufficient to provide the text location information needed for processing in many domains. For example, in the realm of scene text editing, the need to transform text within an image while preserving its style necessitates a level of text shape extraction that point annotation alone cannot provide. More detailed text location information is also required for other tasks such as text erasure, text digitization, etc. These problems prevented the extension of point annotation to more generalized situations.

% Therefore, the motivation for this work is to design a framework for achieving accurate text box prediction from single-point annotations. This framework aims to strike a balance between the acquisition of detailed text location data and the control of annotation costs.

% This work introduces TBSP, which stands for generating Text Boxes from a Single Point, for Scene Text Detection. Given an input image, the text prediction centroids are obtained by SPTS~\cite{peng2022spts}. Subsequently, the PCAG schedule adaptively generates multiple anchors based on the input image size. The optimal anchors are selected based on the confidence of the recognition results in the subsequent training. Following this, the resulting anchors are simultaneously input to the RLPG schedule and RAPR schedule. The RLPG schedule preliminarily aligns the boundary points of the prediction frames with the text through the Thin-Plate Spline transform. Based on the rectification network framework proposed by ASTER~\cite{shi2018aster}, the RLPG schedule can be trained purely by the gradients back propagated by the recognition network, hence requiring no human annotations. Meanwhile, the RAPR schedule uses the attention map to obtain horizontal attention boundaries during the recognition process uses the attention boundaries as a threshold to truncate the predicted boundary points that are beyond the range of the text, and uses the remaining boundary points to draw the minimum horizontal outer moment as the final prediction result.

% Our main contributions can be summarized as follows. 
% \begin{enumerate}
%     \item  For the first time, we successfully trained a scene text detector for generating frames using predictive dot-points from SPTS~\cite{peng2022spts}. It is proved that the localization of text using point annotations is sufficient.

%      \item We propose a boundary point correction mechanism guided by an attention map, which does not require additional training and successfully improves the accuracy of predicting text boxes without increasing the training cost.

%      \item Validate the effectiveness on a wide range of datasets?
% \end{enumerate}


% \section{Related Work}
% \mx{Do we need specific details of some methods here?}

% \textbf{The trends in text detection.} In recent years, the field of scene text detection has progressed through distinct stages of development. From the 1990s to 2010, the primary focus was on horizontal text detection, which used horizontal rectangles for annotation~\cite{karatzas2013icdar,tian2016detecting,liao2017textboxes}. With technological advancements, existing methods achieved excellent performance in detecting horizontal text. Subsequently, from 2010 to 2017, the focus shifted towards multi-oriented text detection, where researchers utilized quadrilaterals for annotation~\cite{karatzas2015icdar,zhou2017east,liu2017deep,liao2018textboxes++,liu2019omnidirectional,tang2019seglink++}. The challenges associated with detecting multi-oriented text were gradually overcome, leading to significant advancements in this area. As progress continued, researchers redirected their efforts toward tackling the intricacies of arbitrarily shaped text~\cite{liu2020abcnet,liu2021abcnetv2,liao2020real,liao2022real,wang2019shape,wang2019efficient}, which necessitated the use of polygons for annotation. As text shapes became more complex, the cost of annotation steadily increased. 

% \textbf{The need for detailed annotation.} Some researchers have begun to explore reducing the cost of annotation~\cite{bartz2018see,hu2017wordsup,tian2017wetext,wupolygon}. They either use fewer samples to achieve competitive performance or use the box to generate the polygon. However, the costly bounding box annotations are still required by both methods.

% Therefore, some methods~\cite{peng2022spts,liu2023spts} aim to reduce annotation costs by employing a single point, which has shown significant success in end-to-end text spotting. However, it's important to note that while a single point is effective in end-to-end text spotting, the bounding box remains crucial for numerous downstream tasks, as emphasized in~\cite{kil2023towards}. Drawing inspiration from previous works~\cite{shi2016robust,shi2018aster,luo2019moran,huang2022swintextspotter,huang2023estextspotter}, utilizing recognition information can greatly assist in the detection process. In this paper, we introduce Point2Polygon, a novel approach that shifts from using individual points to generating polygons. To the best of our knowledge, Point2Polygon is the first scene text detector that generates polygons solely based on a single point and text content.

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/pipeline.png}
%     \caption{ Overview of the proposed model.
%     }
%     \label{fig:related}
% \end{figure*}

% \section{Methodology}
% In this paper, we present a new approach that shows that point-localized text information can efficiently generate polygons for text localization tasks. The overall pipeline is shown in Fig.~\cite{fig:framework} The proposed model consists of three parts. In the following sections, we first describe the three parts in Section 3.1、 3.2 and 3.3 respectively. Then, we describe the training strategy in Section 3.4.

% \subsection{Recognition Confidence Guided Anchor Generation schedule}
% RCAG schedule intercepts anchors from the input image using the text center points predicted by the text center point detector and uses the anchor with the highest recognition confidence in the subsequent recognition network as the optimal anchor. The specific flow of the experiment is explained here with SPTS as the center point detector.

% The text anchor generation is a key step in TPSP. Unlike general objects, text tends to have a more variable size and aspect ratio. Therefore, we include a "long" default box for large aspect ratios, a "short" default box for small aspect ratios, and a normal default box for moderate aspect ratios, all of which are set to multiple sizes to accommodate different text according to the size of the image. Specifically, we resize the aspect ratio of the image to between one-point-three and two, with the exact size determined by the preset value during SPTS training, and set four sizes of normal default boxes, three sizes of long default boxes, and three sizes of short default boxes. Let the size of the image input to the network be (w, h), then the size of the box is determined by the following formula:
% $$
% \begin{aligned}
% & \left(w_l, h_l\right)=\left(\frac{w}{5 \cdot i}, \frac{h}{5 . j}\right) \quad  \\
% & \left(w_s, h_s\right)=\left(\frac{w}{5 . j}, \frac{h}{5 . i}\right) \\
% & \left(w_n, h_n\right)=\left(\frac{w}{10 k} \cdot \frac{h}{10 k}\right) \\
% & i=1.2.3 \quad j=2.3.4 \quad k=1.2.3.5
% \end{aligned}
% $$
% In the subsequent step, we input the boxes into the recognition network for text recognition and calculate the confidence level of the resulting text:
% $$
% P=\sum_i^n P_i / n
% $$
% where $n$ is the length of the text and $P_{i}$ is the prediction confidence for each text

% We select the preset box with the highest confidence level as the optimal box for the text.

% \subsection{Recognition Loss Guided Polygon Generation schedule}
% RLPG schedule supervises the prediction of text boundary points in anchor frames by identification loss. We use the Thin-Plate-Spline (TPS)~\cite{bookstein1989principal} transform to predict boundary points.

% In scene images, text can be rendered in a variety of shapes, but they still morph from the basic rectangle. We first preset 10 equally spaced points on the upper and lower boundaries of the anchor, from which a regular rectangle is formed. We try to establish a mapping between arbitrary text shapes and regular rectangles, so as to realize arbitrary shape text representation. We apply TPS as a basic model to map rectangular preset points to arbitrarily shaped text. This involves obtaining a correspondence for each coordinate from a rectangle to an arbitrary shape. We will refer to the target shape of the text as U and the predefined rectangle as According to the TPS transform, the corresponding point of $(x,y)∈U$ on $S$ can be calculated by
% $$
% \begin{aligned}
% & x^{\prime}=\Phi_x(x, y)=c_x+a_{1_x} x+a_{2_x} y+\sum_{i=1}^k w_{i_x} r\left(d_i\right) \\
% & y^{\prime}=\Phi_y(x, y)=c_y+a_{1_y} x+a_{2_y} y+\sum_{i=1}^k w_{i_y} r\left(d_i\right)
% \end{aligned}
% $$
% where $r$ is the radial basis function

% $
% \begin{aligned}
% & d_i=\left\|(x, y)-\left(x_i, y_i\right)\right\|_2 \\
% \end{aligned}
% $
% is the distance from $(x,y)$ to $(xi,yi)$. ${(x_{1},y_{1}),(x_{2},y_{2}), ..., (x_{k}, y_{k})}$are fixed points on the target shape U, called datums, and k is the number of datums. Given the datum points, the basis function is defined as
% $$
% \begin{aligned}
% & \phi(x, y)=\left[\begin{array}{llllll}
% 1 & x & y & r\left(d_1\right) & \ldots & r\left(d_k\right)
% \end{array}\right]^{\mathrm{T}}
% \end{aligned}
% $$
% then the TPS transform function is determined by the parameters
% $$
% \begin{aligned}
% & \mathrm{T}=\left[\begin{array}{cccccc}
% c_x & a_{1_x} & a_{2_x} & w_{1_x} & \ldots & w_{k_x} \\
% c_y & a_{1_y} & a_{2_y} & w_{1_y} & \ldots & w_{k_y}
% \end{array}\right] 
% \end{aligned}
% $$
% with the shape of $2×(k+3)$.

% Using the TPS transform function, the predefined points on S can be corresponded to the target boundary points on U. The boundary of the text is obtained naturally, like the one demonstrated in Fig. ().
% Inspired by aster[], we similarly use a modified STN[] for modeling spatial transformations as learnable network layers, with subsequent recognition networks to supervise the learning of the locations of target boundary points on U.

% \subsection{Recognition Attention-guided Polygon Refination schedule}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.9\linewidth]{fig/attn.png}
%     \caption{Attention Weight Generation Module.
%     }
%     \label{fig:framework}
% \end{figure}

% Since the observation of the results reveals that the boundary points predicted by the RLPG schedule generally exceed the text, we design the RAPR schedule for obtaining the ATTENTION MAP of the anchors and truncating the predicted boundary points that exceed the text.

% We utilize the Attentional Sequence-to-Sequence Model in the recognition network to obtain the decoder output for each decoding time step while preserving its attention weights $a_{ti}$

% $$
% \begin{aligned}
% & e_{t,i}=\mathbf{w}^{\boldsymbol{\top}} \tanh \left(\mathbf{W} \mathbf{s}_{t-1}+\mathbf{V h}_i+b\right) \\
% & \alpha_{t, i}=\exp \left(e_{t, i}\right) / \sum_{i^{\prime}=1}^n \exp \left(e_{t, i^{\prime}}\right) 
% \end{aligned}
% $$

% $w$, $W$, $V$ are trainable weights.

% The attention weights effectively indicate the importance of each item in the encoder output. We set the attention weights for each step to 1 for attention values greater than a certain threshold and 0 for the remainder. After the recognition is complete, we accumulate the processed single-step weights in the time-step dimension to obtain the complete attention distribution of the anchor:

% $$
% \begin{aligned}
% & \alpha_{t, i}^{\prime}=1 or 0 \\
% & \mathbf{g}_t=\sum_{i=1}^n \alpha_{t, i}^{\prime}
% \end{aligned}
% $$

% We intercepted the prediction boundary points between the largest and smallest horizontal coordinates where the attention value is not 0 as the final prediction boundary points based on the analysis of the attention distribution.

% Finally, we compute the minimum horizontal external moments using the eligible boundary points to obtain the final bounding box and evaluate it.

% \subsection{Training}
% We refer here to aster's bidirectional decoder recognition network for training to demonstrate the effectiveness of the methodology. The model is trained end to end under a multi-task setting, whose objective is

% $$
% \begin{aligned}
% & L=-\frac{1}{2} \sum_{t=1}^T\left(\log p_{\operatorname{ltr}}\left(y_t \mid I\right)+\log p_{\mathrm{rtl}}\left(y_t \mid I\right)\right)
% \end{aligned}
% $$

% where $y_{1},...,y_{t},...,y_{T}$ is the groundtruth text represented by a character sequence.$I$ denotes the input image.

% The objective is the average of the losses on the left-to-right decoder and the right-to-left decoder, whose predicted distributions are denoted by $p_{ltr}$ and $p_{rtl}$, respectively.

% \section{Experiments and Results}


% \section{Conclusion}
% \mx{To Do}

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
